On the Complexity of Opinions and Online Discussions

In an increasingly polarized world, demagogues who reduce complexity down to simple arguments based on emotion are gaining in popularity. Are opinions and online discussions falling into demagoguery? In this work, we aim to provide computational tools to investigate this question and, by doing so, explore the nature and complexity of online discussions and their space of opinions, uncovering where each participant lies. More specifically, we present a modeling framework to construct latent representations of opinions in online discussions which are consistent with human judgements, as measured by online voting. If two opinions are close in the resulting latent space of opinions, it is because humans think they are similar. Our modeling framework is theoretically grounded and establishes a surprising connection between opinions and voting models and the sign-rank of a matrix. Moreover, it also provides a set of practical algorithms to both estimate the dimension of the latent space of opinions and infer where opinions expressed by the participants of an online discussion lie in this space. Experiments on a large dataset from Yahoo! News, Yahoo! Finance, Yahoo! Sports, and the Newsroom app suggest that unidimensional opinion models may often be unable to accurately represent online discussions, provide insights into human judgements and opinions, and show that our framework is able to circumvent language nuances such as sarcasm or humor by relying on human judgements instead of textual analysis.

==> 50background.tex <==
% The problem of information diffusion has been addressed before by studying cascading network on Twitter~\cite{gomez2011uncovering, gomez2010inferring}.
%
% The networks in this case did not model the polarity of the relationship between users.
%
% The problem of generating a signed network has also been studied in depth.

Our work builds upon ideas from several areas of research, viz. (i) opinion mining, (ii) voting models, and (iii) sign-rank estimation. % complexity and recovery.
%
We will discuss related work in each area separately.

% Our work relates two different areas of research and we will identify related work in both areas separately.

\xhdr{Opinion mining}
%
One of the first theoretical models of opinion dynamics and opinion formation is by DeGroot~\cite{degroot1974reaching}, which decided to represent opinions as single real numbers. Since then,
this has been a common modeling choice in many theoretical models of opinions~\cite{axelrod1997dissemination, hegselmann2002opinion, holme2006nonequilibrium, yildiz2013binary, yildiz2010voting}.
However, this modeling choice is in conflict with voting data, which requires multidimensional models of opinions, as argued previously.

% Representing opinions as a single real was a modeling assumption made in the seminal work of~\citet{degroot1974reaching} and it has been a common feature of several opinion models since.
%
%
% De~\ea{} have recently used real valued opinions extracted using NLP tools from Twitter and Reddit posts made by users~\cite{de2014learning}.
%
% Previous work on Memetracker dataset used \emph{memes}, \ie, quotes which were verbatim copied from one article to another, to link articles and have analysed the sentiments in the \emph{context} surrounding the
% meme to determine the nature of relationship among the blogs.
%
% However, NLP tools often are too coarse grained to capture subtleties of language. Also, these techniques do not leverage the input provided by voters acting as oracles.
%
Empirical studies of opinions have often relied on sentiment analysis based on feature extraction methods to measure the po\-la\-ri\-ty of expressed opinions and then determine
the level of agreement between users~\cite{de2016learning, pang2008opinion}.
%
However, it has been also argued that feature extraction methods may be not sufficient to reliably determine the polarity of expressed opinions in several scenarios~\cite{pang2008opinion}.
%
In our work, we overcome this limitation by leveraging the input of voters, acting as \emph{oracles}, to determine the level of agreement (disagreement) between users.

%  \citet[See Section~3.2]{pang2008opinion} have given several examples where standard feature extraction methods will not be sufficient for determining the polarity of the expressed opinions.
%
% In our work, we have utilized the input of voters, acting as oracles, to uncover the relative opinions of comments.

The voting data we work with---upvotes and downvotes between voters and comments---can also be represented as signed graphs, which have been
the focus of several empirical studies in the opinion mi\-ning literature~\cite{akoglu2014quantifying, garimella2018quantifying, leskovec2010predicting, leskovec2010signed}, however, such studies did not consider the existence of underlying multidimensional, multi-sided opinions.
%
In this context, the work by Hsieh \ea~\cite{hsieh2012low} is perhaps more closely related to ours since they aim to uncover the low rank structure of signed graphs via matrix
factorization. That being said, our work differs from their in two key aspects: (i) it explores a novel connection between the factorization of a signed graph and the
sign-rank of a matrix and (ii) it considers that there is an underlying opinion model which is responsible of generating the signed graph.

% The up and downvotes can also be interpreted as creating a bi-partite signed graph between voters and comments.
 %
% Measuring relative agreement/disagreement between comments can also be looked at as predicting the edges of a signed network.
%
% \citet{leskovec2010predicting} use logistic regression and several features extracted from the neighborhood of nodes which are relevant for status theory~\cite{leskovec2010signed} and balance
%. theory~\cite{cartwright1956structural} of social relationships to predict signed edges in networks.
%
% More recently, \citet{tsourakakis2017predicting} have extended the feature set by adding breath first search based heuristic which uses extended paths of signed edges among nodes.
%
% \citet{garimella2018quantifying} have looked at quantifying controversy in online conversations by partitioning the conversation graph on networks like Twitter.
%
% They develop a controversy score for topics using random walks on the graph, but acknowledge that identifying multi-sided controversies as a limitation of their method.
%
% \citet{akoglu2014quantifying} also have designed metrics for measuring controversy on signed bipartite graphs, but have considered only uni-dimensional left/right party leanings.
%
% These methods do not produce a representation of the opinions of the nodes which lead to the disagreement.
%
% \citet{hsieh2012low} have worked on uncovering low rank structure of signed graphs via matrix factorization which is closer to our work.
%
% However, though they make some observations about the signed adjacency matrix being of low rank assuming graph is ``weakly'' balanced in the sense that there are no triads with two positive and one negative edge,
% they do not explore the connections of the factorization to sign-rank of the adjacency matrix.
%
% In our case, we have a bipartite graph of voters and comments and our assessment of relative agreement has been done by crowd-sourced

% sentiment analysis to determine whether a meme, \ie, a quote, had been used in a positive or negative (sentiment) context~\cite{miller2011sentiment}.
%
% and makes the input of voters, acting as oracles, even more important.
%

\xhdr{Voting models}
%
As voting is one of the basic tenets of a democratic society, there is a long history of voting models in the political science and law literature.
% Voting has been studied extensively in political-science and in law as it is one of the basic tenets of a democratic society.
%
However, the majority of voting models in this literature use a single real number to represent political orientation, \ie, left and right leanings~\cite[see references in
Section 4.1.4]{pang2008opinion}. In this context, multidimensional representations of policies have been argued against by favoring the desirable properties of
unidimensional spatial voting models~\cite{rowley1984relevance}.
%
That being said, the Downsian Proximity model and Directional model~\cite{enelow1984spatial, merrill1999unified} can be extended to multidimensional representations.
However, this literature assumes the (policy) dimensions to be known and primarily aims to uncover the relative \emph{weight} that voters give to various policy dimensions.
%
In contrast, in our work, we address the inverse problem of determining the dimension of the multidimensional representations of opinions given the votes cast by the voters.

% \manuel{the related work below is perhaps a bit far away and I would suggest we skip it}
%
% Crowd-sourced clustering approaches take user annotations or judgements about similarity of items to cluster the users or the items.
%
% \citet{yi2012semi} use crowd-sourced similarity measures to do metric-learning for the underlying data and a Bayesian model for the crowd-annotation process was proposed in~\citet{welinder2010multidimensional}.
%
% Recently, \citet{mazumdar2016clustering} have look at the theoretical bounds on the number of active queries needed for uncovering two clusters of nodes which have +1 edges between nodes within the cluster and -1
% between nodes outside the cluster, which maps to uni-dimensional opinion modeling.
%
% Similarly, \citet{vinayak2016crowdsourced} have explored the benefits of asking users for three-item similarity queries, which they refer to as triangular queries.
%
% In our work, the voters implicitly provided us with a multi-way comparison of comments and we have developed a method for leveraging that data.

%  (can be future work once we extract features from the comment texts).
% \citet{cheng2014community} have investigated how community feedback in form of up/down votes shapes user behavior.
  %
%   We will also use the votes given by users but instead of determining how the feedback effects other commenters, we are interested in the latent signal in the voting patterns to help us uncover the underlying network
% between users.

\xhdr{Matrix sign-rank}
%
The notion of sign-rank of a matrix was introduced in the seminal work by Paturi \ea{}~\cite{paturi1984probabilistic} in the context of unbounded error communication complexity
of protocols given by binary matrices.
%
Since then, there has been a rich history of work on matrix sign-ranks~\cite{alon2016sign, basri2009visibility, bhangale2015complexity,  forster2002linear, lee2009approximation}.
%
In terms of sign-rank estimation, Alon \ea{}~\cite{alon2016sign} have developed a polynomial time $\Ocal(N / \log{N})$ multiplicative approximation algorithm, which has been a source of inspiration
for our minimum sign rank estimation algorithm in Section~\ref{sec:sign-rank}.
%
In terms of sign-rank complexity, Basri \ea{}~\cite{basri2009visibility} and Bhangale \ea{}~\cite{bhangale2015complexity} have shown that while one can determine whether $\signrank{\Sbb} \le 2$ for a given sign
matrix $\Sbb$ in polynomial time, determining whether $\signrank{\Sbb} \leq k$ for $k \geq 3$ is NP-hard.
%
% Finally, ~\citet{forster2002linear} provided bounds on the sign-rank of matrices via the spectral norm
%
% Finally, ery recently,~\citet{bhangale2015complexity} perform a complexity analysis of the sign-rank of a generalized sign-matrix, whose entries can take values from $\left\{ +1, 0, -1 \right\}$,
% however, they do not treat zero as missing data but as an actual value.
%
However, in contrast to our own work, where we consider the sign-rank of partially observed matrices, all previous work has considered the sign-rank of fully observed
matrices.

Finally, sign-rank is only one of many measures of matrix complexity such as rank, trace-norm or max-norm. Srebro \ea{}~\cite{srebro2005rank} give an excellent overview of
various other matrix complexity measures.

% \citet{alon2016sign} have provided a polynomial time algorithm for an $\Ocal(N / \log{N})$ multiplicative approximation of the sign-rank. This algorithm was the inspiration behind
% our algorithm for determining the sign-rank of partially observed sign-matrices.

% \citet{bhangale2015complexity} and \citet{basri2009visibility} have shown that one can determine whether $\signrank{\Sbb} \le 2$ for fully observed sign matrix $\Sbb$ in polynomial time.

% Note that \citet{bhangale2015complexity} present results about hardness of determining the sign-rank for a \emph{generalized sign-matrix}, which has entries from $\left\{ +1, 0, -1 \right\}$.
%
% However, they do not treat $0$ as missing data but as an hard equality constraint on the underlying real matrix.

% One bit matrix completion is a classical problem which has been addressed extensively in the literature under various constraints and using different convex
% relaxations~\cite{cai2013max,davenport20141,bhaskar20151}.
%
% We use a variant of solving the problem which takes inspiration from~\citet{bhaskar20151}.
%

%

%
% as the minimum dimension of unbounded error communication complexity
%
% \item \citet{paturi1984probabilistic} proved that for two parties to calculate a function $F: \{0,1\}^n \times \{0,1\}^n \rightarrow \left\{ 0, 1 \right\}$ with probability of error $< \frac{1}{2}$, who each have one of the two $n$ bit numbers, the number of bits which need to be communicated is of the order of the logarithm of the sign-rank of an $2^n \times 2^n$ matrix $\Fb$ where $\Fb_{i,j} = F(i_{\text{binary}}, j_{\text{binary}})$.
%

%
%\citet{forster2002linear} provided bounds on the sign-rank of matrices via the spectral norm and it was shown by \citet{basri2009visibility} and \citet{bhangale2015complexity} that determining whether $\signrank{\Sbb}
% \ge 3$ for a given fully observed sign matrix $\Sbb$ is NP-hard.
%
% \manuel{move to future work the sentence below}
% \red{The hardness result can be easily extended to partially filled matrices. However, the polynomial time algorithm for determining whether a matrix can be embedded in 2D space cannot be easily extended to matrix
% with missing entires?}
%
% Very recently, \citet{alon2016sign} have provided a polynomial time algorithm for an $\Ocal(N / \log{N})$ multiplicative approximation of the sign-rank.
%
% This algorithm was the inspiration behind our algorithm for determining the sign-rank of partially observed sign-matrices.
%
%
% This connection has led to some research in the direction of determining the sign-rank of matrices.
%
%   \item \citet{forster2002linear} discussed bounds on the sign-rank of matrices using the spectral norms which were further improved by \citet{alon2016sign}.
% \begin{equation}
% \signrank{S} \ge \frac{\sqrt{d_1 d_2}}{|| S ||}
% \end{equation}
% where $||S||$ denotes the spectral norm of the matrix.
% \citet{bhangale2015complexity} and \citet{basri2009visibility} have shown that one can determine whether $\signrank{\Sbb} \le 2$ for fully observed sign matrix $\Sbb$ in polynomial time.
%
% \item \citet{bhangale2015complexity} show that determination whether the minimum sign-rank of a full matrix is greater than 3 is NP-hard, though they also present a polynomial algorithm for determining whether the rank of a matrix is less than or equal to 2 (algorithm also presented earlier by~\citet{basri2009visibility}).


%  \item \citet{forster2002linear} proved several lower bounds on the sign rank of the matrix and explored the relationship between $\signrank{\Sbb}$ and the spectral norm of the matrix $\Sbb$. Sign rank of a matrix can also be connected to the existence of large-margin classifiers (see \citet{sherstov2007halfspace} for the connection).

% Note that \citet{bhangale2015complexity} present results about hardness of determining the sign-rank for a \emph{generalized sign-matrix}, which has entries from $\left\{ +1, 0, -1 \right\}$.
%
% However, they do not treat $0$ as missing data but as an hard equality constraint on the underlying real matrix.
%  \item When it comes to matrix completion, the techniques from~\cite{davenport20141}, though theoretically appealing, fail to scale beyond matrices larger than $10^3 \times 10^3$. Hence, we will be using an algorithm which is inspired by the alternating least squares minimization to arrive at a latent representation of the commenters.
  % We will be employing the 1-Bit Matrix completion technique for uncovering the relationships between the users.

